R-SPIDER: A Fast Riemannian Stochastic Optimization Algorithm with Curvature Independent Rate

We study smooth stochastic optimization problems on Riemannian manifolds. Via adapting the recently proposed SPIDER algorithm \citep{fang2018spider} (a variance reduced stochastic method) to Riemannian manifold, we can achieve faster rate than known algorithms in both the finite sum and stochastic settings. Unlike previous works, by \emph{not} resorting to bounding iterate distances, our analysis yields curvature independent convergence rates for both the nonconvex and strongly convex cases.

==> experiments.tex <==
\subsection{Computing the leading eigenvector} \label{sec:experiments-eigenvector}
In this section, we apply our analysis of \rsvrg for gradient dominated functions (Theorem \ref{th:gradient-dominated}) to fast eigenvector computation, a fundamental problem that is still being actively researched in the big-data setting \cite{shamir2015stochastic,garber2015fast,jin2015robust}. For the problem of computing the leading eigenvector, i.e.,
\begin{equation} \label{eq:first-eigenvector}
  \min_{x^{\top}x=1} \quad -x^{\top}\left(\nlsum_{i=1}^n z_iz_i^{\top}\right)x \quad \triangleq \quad -x^{\top} A x = f(x),
\end{equation}
existing analyses for state-of-the-art algorithms typically result in $O(1/\delta^2)$ dependence on the eigengap $\delta$ of $A$, as opposed to the conjectured $O(1/\delta)$ dependence \cite{shamir2015stochastic}, as well as the $O(1/\delta)$ dependence of power iteration.
%\todo{Remove this? Furthermore, the analyses are usually quite non-trivial, either through solving recurrence relations \cite{shamir2015stochastic}, or by an intricate reduction to convex optimization \cite{garber2015fast}.}
% In contrast, we claim that the complexity of (\ref{eq:first-eigenvector}) is indeed $O(1/\delta)$.
Here we give new support for the $O(1/\delta)$ conjecture. Note that  Problem (\ref{eq:first-eigenvector}) seen as one in $\mathbb{R}^d$ is nonconvex, with negative semidefinite Hessian everywhere, and has nonlinear constraints. However, we show that on the hypersphere $\mathbb{S}^{d-1}$ Problem (\ref{eq:first-eigenvector}) is unconstrained, and has \emph{gradient dominated} objective. In particular we have the following result:
%the proof of linear convergence of gradient dominated functions on Riemannian manifolds naturally provide the analysis for an RSVRG algorithm to compute the first eigenvector of a finite sum of PSD matrices. To see this, we prove that the objective function for computing the first eigenvector
%	\[ \min_{x^{\top}x=1} -x^{\top}Ax \]
%is $\tau$-gradient dominated with high probability by random initialization.

\begin{theorem} \label{th:pca-gd}
	Suppose $A$ has eigenvalues $\lambda_1 > \lambda_2 \ge \dots \ge \lambda_d$ and $\delta = \lambda_1 - \lambda_2$, and $x^0$ is drawn uniformly randomly on the hypersphere. Then with probability $1-p$, $x^0$ falls in a Riemannian ball of a global optimum of the objective function, within which the objective function is $O(\tfrac{d}{p^2\delta})$-gradient dominated. 
\end{theorem}


We provide the proof of Theorem \ref{th:pca-gd} in appendix. Theorem \ref{th:pca-gd} gives new insights for why the conjecture might be true -- once it is shown that with a constant stepsize and with high probability (both independent of $\delta$) the iterates remain in such a Riemannian ball, applying Corollary \ref{th:gradient-dominated-corollary} one can immediately prove the $O(1/\delta)$ dependence conjecture. We leave this analysis as future work.

Next we show that variance reduced PCA (VR-PCA) \cite{shamir2015stochastic} is closely related to \rsvrg. We implement Riemannian SVRG for PCA, and use the code for VR-PCA in \cite{shamir2015stochastic}. Analytic forms for exponential map and parallel transport on hypersphere can be found in \cite[Example 5.4.1; Example 8.1.1]{absil2009optimization}. We conduct well-controlled experiments comparing the performance of two algorithms. Specifically, to investigate the dependence of convergence on $\delta$, for each $\delta = 10^{-3} / k$ where $k=1,\dots,25$, we generate a $d\times n$ matrix $Z = (z_1,\dots,z_n)$ where $d=10^3,n=10^4$ using the method $Z=UDV^{\top}$ where $U,V$ are orthonormal matrices and $D$ is a diagonal matrix, as described in \cite{shamir2015stochastic}. Note that $A$ has the same eigenvalues as $D^2$. All the data matrices share the same $U,V$ and only differ in $\delta$ (thus also in $D$). We also fix the same random initialization $x^0$ and random seed. We run both algorithms on each matrix for $50$ epochs. For every five epochs, we estimate the number of epochs required to double its accuracy \footnote{Accuracy is measured by $\frac{f(x) - f(x^*)}{|f(x^*)|}$, i.e. the relative error between the objective value and the optimum. We measure how much the error has been reduced after each five epochs, which is a multiplicative factor $c<1$ on the error at the start of each five epochs. Then we use $\log(2)/\log(1/c)*5$ as the estimate, assuming $c$ stays constant.}. This number can serve as an indicator of the global complexity of the algorithm. We plot this number for different epochs against $1/\delta$, shown in Figure \ref{fig:delta-dependence}. Note that the performance of RSVRG and VR-PCA with the same stepsize is very similar, which implies a close connection of the two. Indeed, the update $\tfrac{x+v}{\|x+v\|}$ used in \cite{shamir2015stochastic} and others is a well-known approximation to the exponential map $\Exp_x(v)$ with small stepsize (a.k.a. retraction). Also note the complexity of both algorithms seems to have an asymptotically linear dependence on $1/\delta$.
\begin{figure}[hbt] 
	\centering
	\includegraphics[width=0.23\linewidth]{figures/pca_result.pdf} \hspace{20pt} \includegraphics[width=0.68\linewidth]{figures/pca_delta.pdf}
	\caption{\small{\bf Computing the leading eigenvector.} Left: RSVRG and VR-PCA are indistinguishable in terms of IFO complexity. Middle and right: Complexity appears to depend on $1/\delta$. $x$-axis shows the inverse of eigengap $\delta$, $y$-axis shows the estimated number of epochs required to double the accuracy. Lines represent different epoch index. All variables are controlled except for $\delta$.} \label{fig:delta-dependence}
\end{figure}


